Adventures in FRET and Specification

This paper gives an overview of previous work in which the authors used NASA's Formal Requirement Elicitation Tool (FRET) to formalise requirements. We discuss four case studies where we used FRET to capture the system's requirements. These formalised requirements subsequently guided the case study specifications in a combination of formal paradigms. For each case study we summarise insights gained during this process, exploring the expressiveness and the potential interoperability of these approaches. Our experience confirms FRET's suitability as a framework for the elicitation and understanding of requirements and for providing traceability from requirements to specification.

==> call.tex <==


https://2024-isola.isola-conference.org/isola-tracks/


Bridging gaps between program specification paradigms (Specify This)
Organizers:

Gidon Ernst (Ludwig-Maximilians-Universität München, DE)
Paula Herber (University of Münster, DE)
Marieke Huisman (University of Twente, NL)
Mattias Ulbrich (Karlsruhe Institute of Technology, DE)
The field of program verification has seen considerable successes in recent years. At the same time, both the variety of properties that can be specified and the collection of approaches that solve such program verification challenges have specialised and diversified a lot. Examples include contract-based deductive specification and verification of functional properties, the specification and verification of temporal properties using model checking or static analyses for secure information flow properties. While this diversification enables the formal analyses of properties that were not accessible a few years ago, it may leave the impression of isolated solutions that solve different isolated problems.

Since Specify This at ISoLa 2022, several efforts have been made towards bridging the gaps between specification and modeling paradigms. This includes coordinated efforts like aDagstuhl seminar as well as community-wide case-studies in the VerifyThis long-term challenge series. The efforts have been very influential in inspiring active research programs, with new theoretical approaches being developed, verification tools gradually embracing more diverse feature sets as part of their specification languages, which in turn unlocks new application areas. In order to maintain momentum and continuity, an upcoming Lorentz seminar is dedicated to discuss further directions on how to increase the expressiveness, abstraction, interoperability, and applications.

The proposed Specify This track at the upcoming ISoLa 2024 will be a perfect and well-timed opportunity by which such fresh ideas on further directions on the integration of specification paradigms can be made concrete:

ISoLa 2024 is intended as the venue in which contributions to the ongoing collaborative VerifyThis long-term challenge are documented and it will offer a similar opportunity for polished solutions to the VerifyThis on-site competition (associated with ETAPS 2024).
Most importantly, we will be able to present and discuss the progress that has been achieved with respect to the perspectives opened up during the Lorentz seminar. There will be new results on approaches that bridge across different specification and verification techniques, including dynamic and static analysis, model checking, deductive verification, security analyses, testing.
